Dirichlet Pruning for Neural Network Compression

We introduce Dirichlet pruning, a novel post-processing technique to transform a large neural network model into a compressed one. Dirichlet pruning is a form of structured pruning that assigns the Dirichlet distribution over each layer's channels in convolutional layers (or neurons in fully-connected layers) and estimates the parameters of the distribution over these units using variational inference. The learned distribution allows us to remove unimportant units, resulting in a compact architecture containing only crucial features for a task at hand. The number of newly introduced Dirichlet parameters is only linear in the number of channels, which allows for rapid training, requiring as little as one epoch to converge. We perform extensive experiments, in particular on larger architectures such as VGG and ResNet (45% and 58% compression rate, respectively) where our method achieves the state-of-the-art compression performance and provides interpretable features as a by-product.

==> tables/table_compression_full.tex <==





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
\begin{table*}
%\small
% \label{tab:table_comp}
    \centering
   % \begin{tabular}{|>{\columncolor[gray]{0.9}}c|c|c|c|c|}
     \begin{tabular}{ccccc}
    \midrule
        %{\rowcolor[gray]{0.9}}
        Method & Architecture & Error & FLOPs & Params\\
        \hline
         \textbf{Dirichlet (50)} & \textbf{39-39-63-48-55-88-87-52-62-22-42-47-47-47}   & 8.6 & \bf{46M} & \bf{0.7M}\\
        
        
        %\hdashline
        
        \textbf{Dirichlet (mean)} & \textbf{34-34-68-68-75-106-101-92-102-92-92-67-67-62-62}  & 8.6 & \bf{46M} & \bf{0.7M}\\
        
        %\hdashline
        % \textbf{IS} & \textbf{39-39-63-48-55-98-97-52}  &  &  & \\ 
        
        %  & \textbf{-62-22-42-47-47-42-62}  & 9.1 & \textbf{34M} & 0.9M\\  \hdashline
        
        %[39, 39, 63, 48, 55, 88, 87, 52, 62, 22, 42, 47, 47, 47, 10]
        
        %./vgg_retrain_filters[25,25,65,80,201,158,165,467,450,490,470,469,469,476,450].1.out:Test Lossds: 0.552 | Acc: 91.160% (9116/10000)
        
        %\hdashline
        
         BC-GNJ & 63-64-128-128-245-155-63-26  -24-24-20-14-12-11-15&  8.3 & 142M & 1.0M\\
         
        
        
        
         %\hdashline
          BC-GHS & 51-62-125-128-228-129-38-13-9-6-5-6-6-20 & 9.0 & 122M & 0.8M\\
          
             
        %\hdashline
        
        RDP  & 27-57-125-122-236-244-246-340-127-77-89-52-380-414&  8.7  & 172M & 3.1M \\ 
              
          \bottomrule
    
    \end{tabular}
    %\vspace{0.5cm}
    \caption{The structured pruning of  \textbf{VGG-16}. Our method using $50$ posterior samples for switches achieved the best compression performance in terms of both FLOPs and the number of parameters with a significantly lower error rate, compared to other existing methods.
    }
    
    \label{tab:compression_rank_vgg}

\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table*}
%\small
% \label{tab:table_comp}
    \centering
   % \begin{tabular}{|>{\columncolor[gray]{0.9}}c|c|c|c|c|}
     \begin{tabular}{ccccc}
    \midrule
        %{\rowcolor[gray]{0.9}}
        Method & Architecture & Error & Comp. Rate & Params\\
        \hline
        
         \textbf{Dirichlet } & \textbf{65,75,70,90,149,149,164,149,305,325,304,306}   & 
         4.5 & 52.2\% 
         & \textbf{17.4M}\\
        
        $L_0$ ARM \cite{li2019l_0} & \text{82-75-82-87-164-169-156-161-317-317-317-324}  & 
        4.4 & $49.9\%$
        & 18.3M\\
        
        $L_0$ ARM \cite{li2019l_0} & 75-72-78-78-157-165-131-162-336-325-331-343 & \textbf{4.3} & $49.6\%$ & 18.4M\\
        
         
              
          \bottomrule
    
    \end{tabular}
    %\vspace{0.5cm}
    \caption{The structured pruning of \textbf{WideResNet-28-10}. Compared to $L_0$-ARM, with a slight increase in the error rate, our method achieves the smallest number of parameters. 
    }
    
    \label{tab:compression_rank_wrn}

\end{table*}






%%%%%%%%%%%%%%%%
%TWO LINE

% \begin{table}[t]
% %\small
% % \label{tab:table_comp}
%     \centering
%   % \begin{tabular}{|>{\columncolor[gray]{0.9}}c|c|c|c|c|}
%      \begin{tabular}{ccccc}
%     \midrule
%         %{\rowcolor[gray]{0.9}}
%         Method & Architecture & Error & FLOPs & Params\\
%         \hline
%          \textbf{IS (50)} & \textbf{39-39-63-48-55-88-87-52}  &  &  & \\
        
%           & \textbf{-62-22-42-47-47-47}  & \textbf{7.9} & \textbf{38M} & \textbf{0.3M}}\\
          
        
%         \hdashline
        
%         \textbf{IS (mean)} & \textbf{34-34-68-68-75-106-101-}  &  &  & \\
        
%           & \textbf{-92-102-92-92-67-67-62-62}  & 8.6 & 46M & 0.7M}\\
        
%         \hdashline
%         % \textbf{IS} & \textbf{39-39-63-48-55-98-97-52}  &  &  & \\ 
        
%         %  & \textbf{-62-22-42-47-47-42-62}  & 9.1 & \textbf{34M} & 0.9M\\  \hdashline
        
%         %[39, 39, 63, 48, 55, 88, 87, 52, 62, 22, 42, 47, 47, 47, 10]
        
%         %./vgg_retrain_filters[25,25,65,80,201,158,165,467,450,490,470,469,469,476,450].1.out:Test Lossds: 0.552 | Acc: 91.160% (9116/10000)
        
%         \hdashline
        
%          BC-GNJ & 63-64-128-128-245-155-63-26&  &  &\\
         
%             & -24-24-20-14-12-11-15& 8.3 & 142M & 1.0M\\
        
        
%          \hdashline
%           BC-GHS & 51-62-125-128-228-129-38-13 &  &  & \\
          
%               & -9-6-5-6-6-20 & 9.0 & 122M & 0.8M\\
%         \hdashline
        
%         RDP  & 27-57-125-122-236-244-246& &  &  \\
%          & -340-127-77-89-52-380-414&  8.7  & 172M & 3.1M \\      
%           \bottomrule
    
%     \end{tabular}
%     %\vspace{0.5cm}
%     \caption{The structured pruning of  VGG-16. Our method using $50$ posterior samples for switches achieved the best compression performance in terms of both FLOPs and the number of parameters with a significantly lower error rate, compared to other existing methods.
%     }
    
%     \label{tab:compression_rank_vgg}

% \end{table}




==> tables/table_compression_full1.tex <==
\begin{table}
%\small
% \label{tab:table_comp}
    \centering
    %\begin{tabular}{|>{\columncolor[gray]{0.9}}c|c|c|c|c|}
    \begin{tabular}{ccccc}
    \toprule
            %{\rowcolor[gray]{0.9}}

        Method & Architecture & Error & FLOPs & Params\\
  	\midrule
          \textbf{Dirichlet (150)} &\textbf{6-8-40-20}&  1.1 & 168K & \textbf{6K} \\ 
          
          \textbf{Dirichlet (mean)} &\textbf{5-8-45-15}&  1.1 & 140K & \textbf{5.5K} \\ 
          
          \textbf{Dirichlet (joint)} &\textbf{6-7-35-17}&  1.1 & 158K & \textbf{5.5K} \\ 
          %RDP &4-7-110-66&  1.0\%} \\
        
          BC-GNJ & 8-13-88-13&  1.0 & 288K & 15K\\ 
          BC-GHS & 5-10-76-16 & 1.0 & 159K & 9K\\ 
          
          RDP & 4-7-110-66 & 1.0 & 117K & 16K\\  
          FDOO (100K) & 2-7-112-478&  1.1 &  \textbf{113K} & 63K \\ 
          %(100K) & & & & \\
          FDOO (200K) & 3-8-128-499& 1.0 & 157K & 76K\\ 
        %(200K) & & & & \\
           GL & 3-12-192-500&  1.0 & 211K & 112K\\ 
           GD & 7-13-208-16&  1.1 & 273K & 29K\\ 
            SBP & 3-18-284-283& \textbf{0.9} & 226K & 99K \\
        \bottomrule
        % {\rowcolor[gray]{0.9}}
        % Method & Architecture & Error & FLOPs & Params\\
        % \hline
        %  \textbf{IS (50)} & \textbf{39-39-63-48-55-88-87-52}  &  &  & \\
        
        %   & \textbf{-62-22-42-47-47-47}  & \textbf{7.9} & \textbf{38M} & \textbf{0.3M}}\\
          
        
        % \hdashline
        
        % \textbf{IS (mean)} & \textbf{34-34-68-68-75-106-101-}  &  &  & \\
        
        %   & \textbf{-92-102-92-92-67-67-62-62}  & 8.6 & 46M & 0.7M}\\
        
        % \hdashline
        % % \textbf{IS} & \textbf{39-39-63-48-55-98-97-52}  &  &  & \\ 
        
        % %  & \textbf{-62-22-42-47-47-42-62}  & 9.1 & \textbf{34M} & 0.9M\\  \hdashline
        
        % %[39, 39, 63, 48, 55, 88, 87, 52, 62, 22, 42, 47, 47, 47, 10]
        
        % %./vgg_retrain_filters[25,25,65,80,201,158,165,467,450,490,470,469,469,476,450].1.out:Test Lossds: 0.552 | Acc: 91.160% (9116/10000)
        
        % \hdashline
        
        %  BC-GNJ & 63-64-128-128-245-155-63-26&  &  &\\
         
        %     & -24-24-20-14-12-11-15& 8.3 & 142M & 1.0M\\
        
        
        %  \hdashline
        %   BC-GHS & 51-62-125-128-228-129-38-13 &  &  & \\
          
        %       & -9-6-5-6-6-20 & 9.0 & 122M & 0.8M\\
        % \hdashline
        
        % RDP  & 27-57-125-122-236-244-246& &  &  \\
        %  & -340-127-77-89-52-380-414&  8.7  & 172M & 3.1M \\      
        %   \hline
    
    \end{tabular}
    %\vspace{0.5cm}
    \caption{The structured pruning of \textbf{LeNet-5}. The pruned network is measured in terms of the number of FLOPs and the number of parameters (Params). We benchmark our method (IS) against RDP~\cite{oh2019radial}, BC-GNJ, BC-GHS~\cite{louizos2017bayesian}, FDOO (100K,200K)~\cite{tang2018flops}, Generalized Dropout (GD)~\cite{srinivas2015data}, Group Lasso (GL)~\cite{wen2016learning}, 
    Structured Bayesian Pruning (SBP)~\cite{neklyudov2017structured}.
    In terms of the number of remaining parameters, our method outperforms other existing methods. 
    }
    
    \label{tab:compression_rank}

\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
